PreRoutGNN for Timing Prediction with Order Preserving Partition: Global Circuit Pre-training, Local Delay Learning and Attentional Cell Modeling

Pre-routing timing prediction has been recently studied for evaluating the quality of a candidate cell placement in chip design. It involves directly estimating the timing metrics for both pin-level (slack, slew) and edge-level (net delay, cell delay), without time-consuming routing. However, it often suffers from signal decay and error accumulation due to the long timing paths in large-scale industrial circuits. To address these challenges, we propose a two-stage approach. First, we propose global circuit training to pre-train a graph auto-encoder that learns the global graph embedding from circuit netlist. Second, we use a novel node updating scheme for message passing on GCN, following the topological sorting sequence of the learned graph embedding and circuit graph. This scheme residually models the local time delay between two adjacent pins in the updating sequence, and extracts the lookup table information inside each cell via a new attention mechanism. To handle large-scale circuits efficiently, we introduce an order preserving partition scheme that reduces memory consumption while maintaining the topological dependencies. Experiments on 21 real world circuits achieve a new SOTA R2 of 0.93 for slack prediction, which is significantly surpasses 0.59 by previous SOTA method. Code will be available at: https://github.com/Thinklab-SJTU/EDA-AI.

==> table/TimingGCN_and_pretrained_encoder.tex <==
\begin{table}[!t]
    \centering
    
    % \adjustbox{width=1.0\linewidth}
    {\small
    \begin{tabular}{ll|cc|ccccccccccccc}
        \toprule

\multicolumn{2}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{|c}{MSE ($\downarrow$)} & \multicolumn{2}{|c}{$R^2_{uf}$ ($\uparrow$)}\\
% \multicolumn{2}{c|}{} & TimingGCN & \makecell{TimingGCN \\ + Pre-training} & TimingGCN & \makecell{TimingGCN \\ + Pre-training}\\
\multicolumn{2}{c|}{} & TimingGCN & {+ Pre-training} & TimingGCN & { + Pre-training}\\
\midrule
\multirow{14}{*}{\rotatebox{90}{train}} & BM64 & 3.997 $\pm$ 3.848 & \textbf{0.691 $\pm$ 0.492} & 0.668 $\pm$ 0.252 & \textbf{0.920 $\pm$ 0.070}\\
~ & aes128 & 4.581 $\pm$ 2.470 & \textbf{1.289 $\pm$ 0.901} & -0.055 $\pm$ 0.312 & \textbf{0.095 $\pm$ 0.468}\\
~ & aes256 & 3.238 $\pm$ 1.037 & \textbf{1.089 $\pm$ 0.216} & 0.499 $\pm$ 0.102 & \textbf{0.583 $\pm$ 0.024}\\
~ & aes\_cipher & 0.429 $\pm$ 0.255 & \textbf{0.410 $\pm$ 0.287} & \textbf{0.644 $\pm$ 0.123} & 0.441 $\pm$ 0.289\\
~ & blabla & 3.475 $\pm$ 1.125 & \textbf{2.439 $\pm$ 1.978} & 0.958 $\pm$ 0.013 & \textbf{0.972 $\pm$ 0.019}\\
~ & cic\_decimator & 0.091 $\pm$ 0.040 & \textbf{0.075 $\pm$ 0.051} & 0.963 $\pm$ 0.014 & \textbf{0.967 $\pm$ 0.011}\\
~ & des & 0.856 $\pm$ 0.355 & \textbf{0.223 $\pm$ 0.076} & 0.905 $\pm$ 0.058 & \textbf{0.981 $\pm$ 0.006}\\
~ & genericfir & 0.612 $\pm$ 0.099 & \textbf{0.474 $\pm$ 0.227} & 0.222 $\pm$ 0.123 & \textbf{0.449 $\pm$ 0.171}\\
~ & picorv32a & 1.386 $\pm$ 0.189 & \textbf{1.220 $\pm$ 0.735} & \textbf{0.839 $\pm$ 0.045} & 0.729 $\pm$ 0.262\\
~ & salsa20 & 4.005 $\pm$ 2.107 & \textbf{3.100 $\pm$ 1.912} & 0.792 $\pm$ 0.118 & \textbf{0.903 $\pm$ 0.049}\\
~ & usb & 0.197 $\pm$ 0.112 & \textbf{0.150 $\pm$ 0.088} & 0.934 $\pm$ 0.035 & \textbf{0.950 $\pm$ 0.026}\\
~ & usb\_cdc\_core & 0.185 $\pm$ 0.041 & \textbf{0.094 $\pm$ 0.023} & 0.961 $\pm$ 0.008 & \textbf{0.980 $\pm$ 0.004}\\
~ & wbqspiflash & 0.343 $\pm$ 0.169 & \textbf{0.280 $\pm$ 0.106} & 0.956 $\pm$ 0.013 & \textbf{0.969 $\pm$ 0.008}\\
~ & zipdiv & 0.370 $\pm$ 0.187 & \textbf{0.177 $\pm$ 0.076} & 0.971 $\pm$ 0.011 & \textbf{0.986 $\pm$ 0.005}\\
\midrule
\multirow{7}{*}{\rotatebox{90}{test}} & aes192 & 4.000 $\pm$ 1.328 & \textbf{0.926 $\pm$ 0.242} & 0.384 $\pm$ 0.205 & \textbf{0.654 $\pm$ 0.097}\\
~ & jpeg\_encoder & 3.950 $\pm$ 1.208 & \textbf{1.511 $\pm$ 0.807} & 0.478 $\pm$ 0.131 & \textbf{0.505 $\pm$ 0.268}\\
~ & spm & 0.220 $\pm$ 0.096 & \textbf{0.065 $\pm$ 0.024} & 0.802 $\pm$ 0.083 & \textbf{0.944 $\pm$ 0.020}\\
~ & synth\_ram & 9.302 $\pm$ 2.617 & \textbf{1.796 $\pm$ 0.819} & 0.735 $\pm$ 0.079 & \textbf{0.943 $\pm$ 0.023}\\
~ & usbf\_device & 1.249 $\pm$ 0.339 & \textbf{0.970 $\pm$ 0.302} & 0.347 $\pm$ 0.119 & \textbf{0.525 $\pm$ 0.184}\\
~ & xtea & 3.613 $\pm$ 2.270 & \textbf{1.111 $\pm$ 0.574} & 0.888 $\pm$ 0.062 & \textbf{0.946 $\pm$ 0.026}\\
~ & y\_huff & 0.764 $\pm$ 0.245 & \textbf{0.435 $\pm$ 0.139} & 0.490 $\pm$ 0.146 & \textbf{0.816 $\pm$ 0.046}\\
\midrule
\multicolumn{2}{c|}{Avg. train} & 1.698  & \textbf{0.837} & 0.733  & \textbf{0.781}\\
\multicolumn{2}{c|}{Avg. test} & 3.300  & \textbf{0.974} & 0.589  & \textbf{0.762}\\


\bottomrule
\end{tabular}
}
\caption{
    Slack prediction with MSE and $R_{uf}^2$ are reported. 
    After applying pre-trained graph encoder into TimingGCN, $R_{uf}^2$ improves 29 \%, showing that our pre-trained graph encoder can serve as a plug-and-play module for training.
    }
\label{tab:TimingGCN-pre-training}
\end{table}

==> table/auxiliary_tasks_R2_only.tex <==
\begin{table*}[!t]
    \centering
    
    % \adjustbox{width=1.0\linewidth}
    {\small
    \begin{tabular}{ll|cc|cc|ccccccccccc}
        \toprule



\multicolumn{2}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{2}{|c}{$R^2_{uf}$ slew ($\uparrow$)} & \multicolumn{2}{|c}{$R^2_{uf}$ net delay ($\uparrow$)} & \multicolumn{2}{|c}{$R^2_{uf}$ cell delay ($\uparrow$)}\\
\multicolumn{2}{c|}{} & TimingGCN & PreRoutGNN & TimingGCN & PreRoutGNN & TimingGCN & PreRoutGNN\\
\midrule
\multirow{14}{*}{\rotatebox{90}{train}} & BM64 & 0.938 $\pm$ 0.025 & \textbf{0.989 $\pm$ 0.004} & 0.984 $\pm$ 0.008 & \textbf{0.992 $\pm$ 0.001} & 0.811 $\pm$ 0.158 & \textbf{0.980 $\pm$ 0.010}\\
~ & aes128 & 0.834 $\pm$ 0.058 & \textbf{0.984 $\pm$ 0.003} & 0.972 $\pm$ 0.006 & \textbf{0.987 $\pm$ 0.001} & 0.751 $\pm$ 0.195 & \textbf{0.983 $\pm$ 0.007}\\
~ & aes256 & 0.853 $\pm$ 0.043 & \textbf{0.983 $\pm$ 0.004} & 0.974 $\pm$ 0.006 & \textbf{0.988 $\pm$ 0.001} & 0.742 $\pm$ 0.219 & \textbf{0.983 $\pm$ 0.008}\\
~ & aes\_cipher & 0.865 $\pm$ 0.039 & \textbf{0.977 $\pm$ 0.001} & 0.971 $\pm$ 0.005 & \textbf{0.983 $\pm$ 0.002} & 0.862 $\pm$ 0.070 & \textbf{0.977 $\pm$ 0.002}\\
~ & blabla & 0.907 $\pm$ 0.038 & \textbf{0.982 $\pm$ 0.004} & 0.987 $\pm$ 0.006 & \textbf{0.994 $\pm$ 0.001} & 0.616 $\pm$ 0.321 & \textbf{0.950 $\pm$ 0.018}\\
~ & cic\_decimator & 0.918 $\pm$ 0.033 & \textbf{0.994 $\pm$ 0.003} & 0.987 $\pm$ 0.009 & \textbf{0.997 $\pm$ 0.000} & 0.909 $\pm$ 0.031 & \textbf{0.984 $\pm$ 0.005}\\
~ & des & 0.867 $\pm$ 0.055 & \textbf{0.988 $\pm$ 0.003} & 0.976 $\pm$ 0.005 & \textbf{0.989 $\pm$ 0.001} & 0.946 $\pm$ 0.033 & \textbf{0.993 $\pm$ 0.004}\\
~ & genericfir & 0.927 $\pm$ 0.024 & \textbf{0.982 $\pm$ 0.001} & 0.976 $\pm$ 0.006 & \textbf{0.986 $\pm$ 0.002} & 0.820 $\pm$ 0.118 & \textbf{0.990 $\pm$ 0.004}\\
~ & picorv32a & 0.814 $\pm$ 0.027 & \textbf{0.877 $\pm$ 0.004} & 0.982 $\pm$ 0.005 & \textbf{0.991 $\pm$ 0.001} & 0.837 $\pm$ 0.109 & \textbf{0.972 $\pm$ 0.008}\\
~ & salsa20 & 0.890 $\pm$ 0.031 & \textbf{0.982 $\pm$ 0.003} & 0.983 $\pm$ 0.004 & \textbf{0.991 $\pm$ 0.001} & 0.752 $\pm$ 0.161 & \textbf{0.971 $\pm$ 0.009}\\
~ & usb & 0.932 $\pm$ 0.033 & \textbf{0.995 $\pm$ 0.002} & 0.991 $\pm$ 0.007 & \textbf{0.998 $\pm$ 0.000} & 0.941 $\pm$ 0.030 & \textbf{0.991 $\pm$ 0.003}\\
~ & usb\_cdc\_core & 0.799 $\pm$ 0.030 & \textbf{0.872 $\pm$ 0.003} & 0.982 $\pm$ 0.009 & \textbf{0.993 $\pm$ 0.000} & 0.910 $\pm$ 0.048 & \textbf{0.988 $\pm$ 0.003}\\
~ & wbqspiflash & 0.899 $\pm$ 0.030 & \textbf{0.972 $\pm$ 0.004} & 0.990 $\pm$ 0.006 & \textbf{0.997 $\pm$ 0.000} & 0.844 $\pm$ 0.061 & \textbf{0.972 $\pm$ 0.009}\\
~ & zipdiv & 0.926 $\pm$ 0.018 & \textbf{0.968 $\pm$ 0.002} & 0.989 $\pm$ 0.009 & \textbf{0.998 $\pm$ 0.000} & 0.906 $\pm$ 0.040 & \textbf{0.986 $\pm$ 0.005}\\
\midrule
\multirow{7}{*}{\rotatebox{90}{test}} & aes192 & 0.816 $\pm$ 0.037 & \textbf{0.967 $\pm$ 0.005} & 0.954 $\pm$ 0.010 & \textbf{0.979 $\pm$ 0.001} & 0.702 $\pm$ 0.244 & \textbf{0.975 $\pm$ 0.005}\\
~ & jpeg\_encoder & 0.783 $\pm$ 0.038 & \textbf{0.949 $\pm$ 0.000} & 0.966 $\pm$ 0.004 & \textbf{0.981 $\pm$ 0.001} & 0.636 $\pm$ 0.233 & \textbf{0.947 $\pm$ 0.011}\\
~ & spm & 0.904 $\pm$ 0.017 & \textbf{0.981 $\pm$ 0.001} & 0.920 $\pm$ 0.010 & \textbf{0.940 $\pm$ 0.019} & 0.831 $\pm$ 0.037 & \textbf{0.981 $\pm$ 0.003}\\
~ & synth\_ram & 0.764 $\pm$ 0.042 & \textbf{0.846 $\pm$ 0.073} & 0.929 $\pm$ 0.014 & \textbf{0.974 $\pm$ 0.001} & 0.533 $\pm$ 0.332 & \textbf{0.682 $\pm$ 0.249}\\
~ & usbf\_device & 0.859 $\pm$ 0.023 & \textbf{0.924 $\pm$ 0.005} & 0.968 $\pm$ 0.001 & \textbf{0.970 $\pm$ 0.003} & 0.824 $\pm$ 0.072 & \textbf{0.976 $\pm$ 0.004}\\
~ & xtea & 0.824 $\pm$ 0.072 & \textbf{0.978 $\pm$ 0.002} & 0.944 $\pm$ 0.011 & \textbf{0.963 $\pm$ 0.000} & 0.574 $\pm$ 0.303 & \textbf{0.968 $\pm$ 0.007}\\
~ & y\_huff & 0.880 $\pm$ 0.026 & \textbf{0.896 $\pm$ 0.002} & 0.940 $\pm$ 0.014 & \textbf{0.964 $\pm$ 0.005} & \textbf{0.844 $\pm$ 0.066} & 0.813 $\pm$ 0.118\\
\midrule
\multicolumn{2}{c|}{Avg. train} & 0.883 & \textbf{0.968} & 0.982 & \textbf{0.992} & 0.832 & \textbf{0.980}\\
\multicolumn{2}{c|}{Avg. test} & 0.833 & \textbf{0.934} & 0.946 & \textbf{0.967} & 0.706 & \textbf{0.906}\\







\bottomrule
\end{tabular}
}
\caption{Comparison of other tasks, including prediction of slew, net delay and cell delay.}

\label{tab:auxiliary-tasks}
\end{table*}

==> table/circuit_representation.tex <==
\begin{table}[!t]
    \centering
    
    % \adjustbox{width=1.0\linewidth}
    {\small
        \begin{tabular}{l|cccccc}
             \toprule
             Type & Object in Circuit  & Feature & Dimension \\
             \midrule
             \multirow{7}{*}{node} & \multirow{7}{*}{pin/PI/PO} & primary I/O or not & $1$\\
             ~ & ~ & fan-in or fan-out & $1$\\
             ~ & ~ & distance to boundaries & $4$\\
             ~ & ~ & capacitance & $4$ \\
             ~ & ~ & level encoding & $1 + 2\times 4$\\
             ~ & ~ & node embedding & $4$\\
             ~ & ~ &  graph embedding & $4$\\
             \midrule
             \multirow{3}{*}{edge cell} & \multirow{3}{*}{fan-in to fan-out} & LUT valid or not & $8$ \\
             ~ & ~ & LUT axis & $8 \times (7 + 7)$ \\
             ~ & ~ & LUT values & $8 \times (7 \times 7)$ \\
             edge net & net driver to net sink & relative location & $2$\\
             edge net\_inv & net sink to net driver & relative location & $2$\\
             \bottomrule
        \end{tabular}
    }

    \caption{
    Nodes and edges of circuit heterogeneous DAG. 
    LUTs in cell are designed for output slew and cell delay under four corner conditions, EL/RF. 
    }
    \label{tab:circuit-representation}
\end{table}

==> table/circuit_representation_small.tex <==
\begin{table}[!t]
    \centering
    
    % \adjustbox{width=1.0\linewidth}
    {\small
        \begin{tabular}{l|cccccc}
             \toprule
             Type & Object in Circuit  & Feature  \\
             \midrule
             \multirow{7}{*}{node} & \multirow{7}{*}{pin/PI/PO} & primary I/O or not \\
             ~ & ~ & fan-in or fan-out \\
             ~ & ~ & distance to boundaries \\
             ~ & ~ & capacitance  \\
             ~ & ~ & level encoding \\
             ~ & ~ & node embedding \\
             ~ & ~ &  graph embedding \\
             \midrule
             \multirow{3}{*}{edge cell} & \multirow{3}{*}{fan-in to fan-out} & LUT valid or not \\
             ~ & ~ & LUT axis  \\
             ~ & ~ & LUT values  \\
             edge net & net driver to net sink & relative location \\
             edge net\_inv & net sink to net driver & relative location\\
             \bottomrule
        \end{tabular}
    }

    \caption{
    Nodes and edges of circuit heterogeneous DAG. 
    LUTs in cell are designed for output slew and cell delay under four corner conditions, EL/RF. 
    }
    \label{tab:circuit-representation}
\end{table}

==> table/routing-STA-time.tex <==
\begin{table}[!t]
    \centering
    \adjustbox{width=0.8\linewidth}{
        \begin{tabular}{l|cccccccccccccccccccc}
            \toprule

Circuit & Routing & STA & Total & TimingGCN & PreRoutGNN\\
\midrule
BM64 & 713.000 & 13.600 & 726.600 & 0.291 & 0.319\\
aes128 & 1787.000 & 51.400 & 1838.400 & 0.408 & 0.548\\
aes192 & 1728.000 & 58.600 & 1786.600 & 0.438 & 0.591\\
aes256 & 2886.000 & 72.000 & 2958.000 & 0.432 & 0.623\\
aes\_cipher & 1849.000 & 18.700 & 1867.700 & 0.210 & 0.252\\
blabla & 836.000 & 23.600 & 859.600 & 0.498 & 0.524\\
cic\_decimator & 81.000 & 3.300 & 84.300 & 0.114 & 0.124\\
des & 493.000 & 16.200 & 509.200 & 0.149 & 0.192\\
genericfir & 409.000 & 11.100 & 420.100 & 0.101 & 0.126\\
jpeg\_encoder & 4191.000 & 70.300 & 4261.300 & 0.421 & 0.591\\
picorv32a & 987.000 & 18.500 & 1005.500 & 0.490 & 0.536\\
salsa20 & 1738.000 & 29.100 & 1767.100 & 0.474 & 0.526\\
spm & 14.000 & 4.200 & 18.200 & 0.052 & 0.061\\
synth\_ram & 452.000 & 9.300 & 461.300 & 0.074 & 0.092\\
usb & 45.000 & 3.400 & 48.400 & 0.097 & 0.108\\
usb\_cdc\_core & 3654.000 & 4.700 & 3658.700 & 0.212 & 0.224\\
usbf\_device & 1525.000 & 21.000 & 1546.000 & 0.325 & 0.371\\
wbqspiflash & 181.000 & 5.900 & 186.900 & 0.319 & 0.349\\
xtea & 174.000 & 4.900 & 178.900 & 0.323 & 0.342\\
y\_huff & 1162.000 & 15.400 & 1177.400 & 0.174 & 0.205\\
zipdiv & 48.000 & 3.500 & 51.500 & 0.205 & 0.218\\
\midrule
Avg. & 1188.238 & 21.843 & 1210.081 & 0.277 & 0.330\\



\bottomrule
\end{tabular}
}

\caption{
Execution time recorded with second (s).
% Accurate timing information can be accessed only after routing stage, so we record the routing and STA execution time.
% Note that our method predicts \textbf{post-routing} timing information in \textbf{pre-routing} stage, which means we do not need to implement the timing-consuming routing stage.
% The runtime of our PreRoutGNN is similar to baselines, but we improve the accuracy from 0.58 to 0.93, outperforming other methods with a large margin.
}
\label{tab:routing-STA}
\end{table}
